Verified Scalable Parallel Computing with Why3

BSML is a pure functional library for the multi-paradigm language OCaml. BSML embodies the principles of the Bulk Synchronous Parallel (BSP) model, a model of scalable parallel computing. We propose a formalization of BSML primitives with WhyML, the specification language of Why3 and specify and prove the correctness of most of the BSML standard library. Finally, we develop and verify the correctness of a small BSML application.

==> experiments.tex <==
\fl{In this section we present timing experiments on a
    parallel machine of the application(s) we developped in
    the previous section. It means we also should explain
    how we extracted OCaml code from our \why formalization.}
